A Reconnaissance Attack Mechanism for Fixed-Priority Real-Time Systems

In real-time embedded systems (RTS), failures due to security breaches can cause serious damage to the system, the environment and/or injury to humans. Therefore, it is very important to understand the potential threats and attacks against these systems. In this paper we present a novel reconnaissance attack that extracts the exact schedule of real-time systems designed using fixed priority scheduling algorithms. The attack is demonstrated on both a real hardware platform and a simulator, with a high success rate. Our evaluation results show that the algorithm is robust even in the presence of execution time variation.

==> Makefile <==
# Makefile for Latex
# Created by Sibin M.
# Date : May 15, 2004.

# LATEX = pdflatex 
LATEX = xelatex 
BIBTEX = bibtex
DVIPS = dvips
DVIPDF = dvipdf
PDFTOOO = pdf2oo -batch 
PSTOPDF = ps2pdf
PDFTOPS = pdf2ps
ACROBAT_COMPATIBILITY = 1.5

# MAIN_FILE_NAME = rtss09
MAIN_FILE_NAME = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex | gawk -F . 'BEGIN {filename;} /tex/ { filename = $$1; } END{printf(filename);}' )
BIB_FILES = mybib.bib realime.bib ada9x.bib sibin.bib power.bib zhu.bib arch.bib
# BIB_FILES := $(shell perl -ne '($$_)=/^[^%]*\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $(SRC))

EMBED_SRC := $(MAIN_FILE_NAME)
EMBED_RESULT := $(MAIN_FILE_NAME)_embedded
EMBED = gs -sDEVICE=pdfwrite -q -dBATCH -dNOPAUSE -dSAFER -dPDFX -dPDFSETTINGS=/prepress -dAutoFilterColorImages=false -dColorImageFilter=/FlateEncode -dAutoFilterGrayImages=false -dGrayImageFilter=/FlateEncode -sOutputFile=$(EMBED_RESULT).ps -c '<> setdistillerparams' -f $(EMBED_SRC).ps -c quit

GOALS = $(MAIN_FILE_NAME).dvi

#%.pdf:  %.dvi
#	$(DVIPDF) $<
#	$(EMBED)

%.pdf:  %.ps
#	$(DVIPDF) $<
#	$(EMBED)
#	$(PDFTOPS) $(EMBED_RESULT).pdf 
#	cp $(EMBED_RESULT).ps $(EMBED_RESULT)_temp.ps
	$(EMBED)
	$(PSTOPDF) -dCompatibilityLevel=$(ACROBAT_COMPATIBILITY) -dMAxSubsetPct=100 -dSubsetFonts=true -dEmbedAllFonts=true -sPAPERSIZE=letter $(EMBED_RESULT).ps
	cp $(EMBED_RESULT).pdf $(MAIN_FILE_NAME)_submission.pdf


%.ps:	%.dvi
	$(DVIPS) -o $(MAIN_FILE_NAME).ps $<

%.odp:	%.pdf
	$(PDFTOOO) $(MAIN_FILE_NAME).pdf

%.dvi:	$(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

all: 	clean $(GOALS)

$(MAIN_FILE_NAME).dvi:	$(MAIN_FILE_NAME).tex
	$(LATEX) $(MAIN_FILE_NAME)
	$(BIBTEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)
	$(LATEX) $(MAIN_FILE_NAME)

clean:
	rm -rf *.dvi *.log *.bbl *.blg *.aux *~

clobber:
	make clean
	rm -rf $(MAIN_FILE_NAME).pdf $(MAIN_FILE_NAME).ps $(MAIN_FILE_NAME).odt


==> discussion_future_work.tex <==
\section{Discussion}
\label{discussion}

We evaluated the algorithm by varying four variables: \ci execution time variation, \cii CPU utilization, \ciii the number of tasks \civ observed duration. 
From the results, we can conclude that 
\ca large execution time variation can reduce the precision of the inference;
%adds uncertainty to the schedule and influences the inference performance;
\cb having more tasks in a system means more possible combinations in decomposing a busy interval;
%adds more complexity to the schedule;
%the factors influencing the precision of our algorithm are:
%\begin{enumerate}
%\ca having harmonic tasks (either partially or entirely) in the task set reduces the precision of the inference; 
%\cb having random initial arrival times adds uncertainty to the schedule; 
\cc a short busy interval reduces the probability that an inferred arrival time can successfully land within the busy interval;
%\cc low utilization implies short and scattered busy intervals, which increases that probability that the \ATTCKNF algorithm can't resolve on an inference;
\cd higher utilization represents larger busy intervals and more tasks involved in one individual busy interval, leading to increased uncertainty;% and lower inference precision;
and \ce accumulating more busy interval observation can improve the inference precision.
%
In the following we discuss the potential impacts of uncertainty or error in attacker's knowledge and of defenses that a system designer might employ.

\noindent
\textbf{Tasks with Variant Execution Modes:}
In this paper, we consider the average execution time $c_i$ and the variation within certain range around $c_i$. 
Particularly, we use normal distribution to generate such variation in our simulation-based evaluation.
However, this single distribution model may not fit tasks that 
can switch between different execution modes, each of which may have a distinct average execution time and variation.
%have diverse branch paths since the actual execution times of such tasks heavily depend on the depth of the path. 
For instance, an image encoder task may 
consist of several modes to support diverse image formats. Each mode in the task implements a distinct image encoder and thus may have varied execution time.

To deal with this issue, rather than using a single average execution time for a task, we could model each mode 
%that has significant variation 
with a separate distribution. 
%The average execution time for such a mode can also be obtained from the corresponding distribution.
In fact, such information is also available during the process of WCET analysis \cite{%wartel2013measurement,
cucu2012measurement}.
As a result, a task may have multiple possible average execution times.
%
To make the \ATTCKNF algorithm tolerate this variation, we could take every mode's average execution time into account when decomposing a busy interval in the second step. Note that having multiple average execution times for a task does not affect the analysis of the arrival window since its period remains unchanged.
%, which is what \ATTCKNF mainly relies on.

\noindent
\textbf{Incomplete Knowledge of Task Set:}
In this paper, we assume that the attacker is capable of obtaining information regarding the system's task set, described in \cref{subsec:attackmodel}. If the attacker only has limited task set information that is insufficient to proceed the decomposition of captured busy intervals, then \ATTCKNF will not be usable.
Nevertheless, the algorithm can easily be adapted to estimating the probability of a task being scheduled in a given interval rather than inferring the exact start time of a victim task. 
%\todo[inline]{$\uparrow$ CY: Make it clear.}

\noindent
\textbf{Variant Observer Task:}
\ATTCKNF utilizes an \OBSERVER to capture busy intervals. If the attacker owns a task $\tau_i$ that is not the lowest priority, it will only be preempted by higher priority tasks $\{\tau_{i+1},...\tau_{n}\}$.
Also, to comply with real-time constraints, such a task must have a fixed period and worst case execution time. Thus observation capability of busy intervals is constrained. Nonetheless, it is still possible to reconstruct the schedule of tasks that have a higher priority than the \OBSERVER, but it increases the risk of being detected while running the \ATTCKNF algorithm because now the execution of the \OBSERVER impacts the lower priority tasks.  
%\todo[inline]{$\uparrow$ CY: Should we clarify the last claim? Who really carries out the attack?}

\input{discussion_scobe}

==> discussion_scobe.tex <==
%\noindent
%\textbf{SCOBE}\\
%\textbf{Scheduling Randomization}\\
\noindent {\bf Dealing with Randomization Defenses:} The schedule reconstruction mechanism in \ATTCKNF leverages the \emph{limited uncertainty} in the repeating schedules generated by a fixed-priority scheduler. Defenders may \emph{randomize} the schedules so that there is no guarantee that the next hyper-period will show the exact same order (and timing) of execution for the tasks~\cite{2016:taskshuffler}. 
%For instance, by picking a random task instead of the one with the highest-priority at each scheduling point, subject to the deadline constraints~\cite{2016:taskshuffler}.
%\todo[inline]{cite RTAS paper} 
%
\begin{comment}
Figure~\ref{fig:diss_random_schedule} shows a part of the schedule for the task set in Example~\ref{ex:Nk_certain} generated by the randomization algorithm. It shows tasks being \emph{shuffled} within each busy interval.  

\begin{figure}[b]
    \vspace{-\baselineskip}
    \centering
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=1.0\columnwidth,height=0.75in]{Figures/RandomScheduling_Normal}
        \vspace{-\baselineskip}
        \caption{No randomization}
        %\vspace{-\baselineskip}
    \end{subfigure}%
    
    \hfill
        
    \begin{subfigure}[t]{0.49\textwidth}
        \centering
        \includegraphics[width=1.0\columnwidth,height=0.75in]{Figures/RandomScheduling_Random}
        \vspace{-\baselineskip}
        \caption{Randomization}
        %\vspace{-\baselineskip}
    \end{subfigure}
    \vspace{-\baselineskip}
    \caption{Partial Schedules with and without the randomization for $10$ hyper-periods.}
    \label{fig:diss_random_schedule}
    \vspace{-\baselineskip}
\end{figure}
\end{comment}
%
% The following is from Amir:
%Suppose a work conserving randomized scheduler is used in the system.
%To inspect the effectiveness of our algorithm against 
%
Such methods can be countered based on the fact that arrival times do not depend on the scheduling policy. 
We can use the arrival window estimations in our algorithm to find such time instances.
Note that if at any instance in time there are many other tasks waiting to be executed, then by the properties of such randomization scheduling, $\STME$ could be at any time in the interval $[\ATME,\ATME+p_i-c_i]$. Therefore, in this case even if $\ATME$ is known, without other information no algorithm can predict $\STME$ accurately.
%
\begin{comment}
To counter such randomization methods, let the arrival time of one instance of task $\tau_i$ be denoted by $\ATME$ and we want to predict its corresponding start time $\STME$. If at any instance in time there are many other tasks waiting to be executed, then by the properties of such randomization scheduling, $\STME$ could be at any time in the interval $[\ATME,\ATME+p_i-c_i]$. Therefore, even if $\ATME$ is known, no algorithm can predict $\STME$ accurately. On the other hand, if we find a time in the busy interval such that $\tau_i$ is the only buffered task and no other task is being executed, then by the work conserving property of the scheduler, $\tau_i$ has to be executed and we choose this point as the latest time for $\STME$. 
Note that arrival times do not depend on the scheduling policy, so they are still of use in the face of randomization.
Thus, we can use the arrival window estimations 
in our algorithm to find such time instances.

We focus on each busy interval and look for the following condition: Suppose for $i\in\{1,...,j\}$ the intervals $\overline{a_i}=[\alpha_i,\beta_i]$ with $\alpha_i\le \alpha_{i+1}$, for $1\le i\le j-1$, are the arrival windows estimated by our algorithm in a given busy interval. If there exists point $x_i\in \overline{a_i}$ such that $x_i > \alpha+\sum_{k < i} c_k$ ($\alpha$ is assumed to be the start point of the busy interval) and $x_i < \alpha_{i+1}$, then we change $\beta_i$ to $x_i$, and hence we can make the arrival window narrower. Due to the work conserving property of the scheduler we understand that $\tau_i$ should have started to be executed by $x_i$. Hence, if we choose the first point of the arrival window as the starting time, the error in estimating the start time will be in the interval $[0,x_i-\alpha_i]$. For instance, for the special case that $\tau_i$ is the only task whose arrival window starts at the beginning of the busy interval (\ie $\alpha=\alpha_i$), we {\em can find the exact starting time} of $\tau_i$. This trick could be also used, when randomization is absent, to improve the accuracy of the estimation of arrival windows. After making arrival window $\overline{a_i}$ narrower by changing $\beta_i$ to $x_i$, we can take its intersection with the arrival window in other segments. Hence, all of them become narrower. This step could be implemented by having a list of ready to execute tasks. If at some point there is only one task in this list and no task is being executed, due to the work conserving property of the scheduler, that task should be executed. So our \ATTCKNF mechanism can even deal with some randomization-based defenses.
\end{comment}

==> measurement.tex <==



==> trigger.tex <==
\section{Triggering Collaborative Attacks}
\label{sec::trigger}

To demonstrate the the feasibility and utility of the proposed schedule reconstruction scheme on a realistic platform, we implemented a targeted cache timing attack on \emph{Zedboard} that leverages provided schedule information. The cache timing attack is implemented in a collaborative compromised task which behaves normally until it receives a signal from the idle task after the schedule is reconstructed.

A cache timing attack utilizes time difference between cache-hit and cache-miss when accessing data via processor's cache to estimate the amount of attacker's data existing in the cache. By knowing how much data is evicted from the cache, an attacker can estimate the cache usage of the victim task and potentially infer its memory usage as well.

In this demonstration, we target a camera task which compresses pictures taken by a camera module. It runs under $30ms$ in period with $10ms$ worst case execution time. The camera task initiates with no-operation mode and starts capturing photos with low resolution by default. It switches to high resolution mode when details need to be captured. The switch between these modes results in a shift in memory usage by the camera task. The goal of our attack from the malicious task, which runs under $10ms$ in period and $2ms$ in worst execution time with priority higher than the camera task, is to detect the switch between the camera modes by monitoring the tasks' cache usage. Such an attack for example could help the attacker identify locations of special interest for an UAV during a reconnaissance mission.    

To launch a cache timing attack, the malicious task must locate the start time of the victim task, which is done by referring to the reconstructed schedules. The idle task then issues a signal to malicious task prior to an execution of the victim task, and the malicious task launches the attack by using Algorithm~\ref{algo:cache_attack}. In traditional enterprise computers or cloud computing settings an adversary may be able to periodically launch the attack till he finds the victim task executing, but in a real-time systems such a strategy might result in missed deadlines for legitimate tasks leading to scrutiny of the system and increased risk of detection for the attacker. 

\begin{algorithm}
\caption{Cache Timing Attack}
\label{algo:cache_attack}
\begin{algorithmic}[1]
\STATE \{$T_{hit}$: \emph{cache access time with all cache-hit} \}
\STATE \{$T_{miss}$: \emph{cache access time with all cache-miss} \}
\STATE \{$T_{victim}$: \emph{cache access time after victim task} \}
\STATE \{\emph{time(CacheRead): measure access time to all cache lines}\}
\STATE {}
%\STATE \textbf{One Time Initialization:}
\STATE \emph{Clear all cache lines}
\STATE {$T_{miss} \leftarrow$ \emph{time(CacheRead)}}
\STATE {$T_{hit} \leftarrow$ \emph{time(CacheRead)}}
\WHILE {\emph{victim task has not ended}}
	\STATE \emph{NOP}
\ENDWHILE
\STATE {$T_{victim} \leftarrow$ \emph{time(CacheRead)}}
\RETURN $(T_{victim}-T_{hit})/(T_{miss}-T_{hit})$
\end{algorithmic}
\end{algorithm}


\todo[inline]{@Reviewer: "The cache attack was demonstrated in the absence of any task that can preempt tha target task, even though "undoubtedly, presence of another task that can preempt the victim would cause some distortion". Since the whole motivation is deadling with complex multi-task scheduling, this detracts from the value of the empirical demonstration."\\

@CY: Explain more about the interpretation of the value of cache timing attack here (we use cache timing attack to learn system behavior but not to get exact memory usage.}

Figure~\ref{fig:cache_attack} presents the inference of the cache usage amount and the memory usage patterns. The results suggest that the transitioning points of the memory usage at sampling count 15, 70 and 90 can be easily observed from the inferred cache usage pattern. Note that, in this demonstration, no other tasks preempted the victim task. Undoubtedly, presence of another task that can preempt the victim would cause some distortion on the cache usage amount. Nevertheless, the pattern will be recognizable in this case since the camera task consumes the most memory, which makes the usage from other tasks subtle and negligible. Furthermore, knowing the schedule could help the attacker account for noise from other tasks. 

\begin{figure}[t]
\vspace{-\baselineskip}
\centering
\includegraphics[width=1\columnwidth,height=2in]{Figures/CacheAttack}
%\vspace{-\baselineskip}
\caption{Cache timing attack over a camera task that shows how the transition of the memory usage (green line) can be recovered by the observation of the cache usage (blue line).}
\label{fig:cache_attack}
\vspace{-1.5\baselineskip}
\end{figure}



